0-1 phase transitions in sparse spiked matrix estimation

We consider statistical models of estimation of a rank-one matrix (the spike) corrupted by an additive gaussian noise matrix in the sparse limit. In this limit the underlying hidden vector (that constructs the rank-one matrix) has a number of non-zero components that scales sub-linearly with the total dimension of the vector, and the signal strength tends to infinity at an appropriate speed. We prove explicit low-dimensional variational formulas for the asymptotic mutual information between the spike and the observed noisy matrix in suitable sparse limits. For Bernoulli and Bernoulli-Rademacher distributed vectors, and when the sparsity and signal strength satisfy an appropriate scaling relation, these formulas imply sharp 0-1 phase transitions for the asymptotic minimum mean-square-error. A similar phase transition was analyzed recently in the context of sparse high-dimensional linear regression (compressive sensing).

==> sections/APP_coverlap_snr.tex <==
\section{Variation of the overlap with the SNR}

\subsection{Proof of \eqref{jacPos}}

 Setting $R=R_n(t,\epsilon)$ and dropping the time index in the Gibbs-bracket we have
%
\begin{align*}
\frac{d\,\EE\langle Q\rangle}{dR}=n\EE\big\langle Q(\langle {\cal L}\rangle-{\cal L})\big\rangle
\end{align*}
where $\cal L$ is given by \eqref{def_L}. $R$ appears both in the numerator and partition function that define the bracket $\langle -\rangle$, thus the difference appearing. This is the same mechanism as when we derived identity \eqref{GaussIPP}. We have already shown in the previous appendix that $-\EE\langle Q{\cal L}\rangle= \EE\langle Q^2\rangle-\frac12\EE[\langle Q\rangle^2]$. It remains to compute
%
\begin{align*}
\EE[\langle Q\rangle \langle {\cal L}\rangle]=\mathbb{E}\Big[\langle Q \rangle\frac{\big\langle \|\bx\|^2 \big\rangle}{2n} -  \langle Q \rangle^2 - \langle Q \rangle\frac{\tilde \bZ \cdot \langle \bx\rangle}{2n\sqrt{R}}  \Big]	\,.
\end{align*}
By formulas \eqref{SteinLemma} and \eqref{GaussIPP} in which the Hamiltonian is \eqref{Ht} we have (here $\nabla\equiv\nabla_{\tilde \bZ}$)
\begin{align*}
-\frac{1}{2n\sqrt{R}}\EE\big[\tilde \bZ \cdot \langle \bx\rangle\langle Q \rangle \big]	&= -\frac{1}{2n\sqrt{R}}\EE\big[\langle Q\rangle \nabla\cdot \langle \bx\rangle + \langle \bx\rangle\cdot \nabla \langle Q\rangle\big]\nn
%
&=-\frac{1}{2n}\EE\big[\langle Q\rangle \big(\big\langle \|\bx\|^2\big\rangle-\|\langle\bx\rangle\|^2\big) + \langle \bx\rangle\cdot \big(\langle Q\bx\rangle-\langle Q\rangle \langle \bx\rangle\big)\big]\nn
%
&\overset{\rm N}{=}-\frac{1}{2n}\EE\big[\langle Q\rangle \big\langle \|\bx\|^2\big\rangle\big]+\frac{1}{n}\EE\big[\langle Q\rangle \|\langle \bx \rangle \|^2\big]-\frac12\EE[\langle Q\rangle^2]\,.
\end{align*}
We used the following consequence of the Nishimori identity. Let $\bx,\bx^{(2)}$ be two replicas, i.e., conditionally (on the data) independent samples from the posterior \eqref{tpost}. Then $$\frac1n\EE\big[\langle \bx\rangle\cdot \langle \bx Q\rangle\big]=\frac1{n^2}\EE\big\langle (\bx^{(2)}\cdot \bx) (\bx\cdot \bX)\big\rangle\overset{\rm N}{=}\frac1{n^2}\EE\big\langle (\bx^{(2)}\cdot \bX) (\bX\cdot \bx)\big\rangle=\EE[\langle Q\rangle^2]\,.$$
We reach
\begin{align*}
\EE\big\langle Q(\langle {\cal L}\rangle-{\cal L})\big\rangle &=	\EE\langle Q^2\rangle-2\EE[\langle Q\rangle^2]+\frac{1}{n}\EE\big[\langle Q\rangle \|\langle \bx \rangle \|^2\big]\nn
&=\frac{1}{n^2}\EE\big\langle(\bx\cdot\bX)^2-2(\bx\cdot\bX)(\bx^{(1)}\cdot\bX)+(\bx\cdot\bX)(\bx^{(2)}\cdot\bx^{(3)})\big\rangle\nn
%
&\overset{\rm N}{=}\frac{1}{n^2}\EE\big\langle(\bx\cdot\bx^{(0)})^2-2(\bx\cdot\bx^{(0)})(\bx^{(1)}\cdot\bx^{(0)})+(\bx\cdot\bx^{(0)})(\bx^{(2)}\cdot\bx^{(3)})\big\rangle
\end{align*}
where $\bx^{(0)},\bx,\bx^{(2)}, \bx^{(3)}$ are replicas. Component-wise and after multiplying by $n$ this gives
%
\begin{align}
\frac{d\,\EE\langle Q\rangle}{dR} &=\frac{1}{n}\sum_{i,j=1}^n\EE\big\langle x_ix_i^{(0)} x_jx_j^{(0)} -2x_ix_i^{(0)}x_j^{(1)}x_j^{(0)}+x_ix_i^{(0)}x_j^{(2)}x_j^{(3)}\big\rangle\nn
%
&=\frac{1}{n}\sum_{i,j=1}^n\EE\big[\langle x_ix_j\rangle^2 -2\langle x_i\rangle \langle x_j\rangle \langle x_ix_j\rangle+ \langle x_i\rangle^2\langle x_j\rangle^2\big]\ge 0 \label{secondDer_f_pos}
\end{align}
which proves \eqref{jacPos}.\\

\subsection{Proof of \eqref{JacUV}}
 Identity \eqref{JacUV} follows from the following inequality that we prove now: $$\frac{\partial \EE\langle Q_V\rangle}{\partial R_V}\ge 0$$


==> sections/APP_stationary_cond.tex <==
\section{Proof of \eqref{boundaries_WS}}
%
Let us show how to obtain the stationary condition \eqref{boundaries_WS}. It follows from the I-MMSE theorem \cite{GuoShamaiVerdu_IMMSE}, but we prove it for completeness. Starting from $\partial_{q} f^{\rm pot}_n(q) = 0$ gives
%
\begin{align*}
q \lambda_n	= 2\frac{d}{dq} \mathbb{E} \ln \int d{P}_0^{(n)}(x) e^{-\big(q\lambda_n\,\frac{x^2}{2}-q\lambda_n\, x X -\sqrt{q\lambda_n}\,x Z\big)}= \lambda_n\mathbb{E}\Big\langle -x^2+2xX+\frac{xZ}{\sqrt{q}}\Big\rangle_q\,.
\end{align*}
%
Now we integrate by part the Gaussian variable using the elementary formula $\mathbb{E}[Zg(Z)]=\mathbb{E}\,g'(Z)$ for $Z\sim {\cal N}(0,1)$ and $g$ a bounded function. This gives $\mathbb{E}[Z\langle x\rangle_q]/\sqrt{q}=\mathbb{E}[\langle x^2\rangle_q-\langle x\rangle_q^2]$. Therefore $$\mathbb{E}\Big\langle -x^2+2xX+\frac{xZ}{\sqrt{q}}\Big\rangle_q = 2\mathbb{E}[X\langle x\rangle_q]-\mathbb{E}[\langle x\rangle_q^2]=\mathbb{E}[X\langle x\rangle_q]$$ using the Nishimori identity, that implies $\mathbb{E}[X\langle x\rangle_q]=\mathbb{E}[\langle x\rangle_q^2]$, for the last equality. 

==> sections/APP_t_der.tex <==
\section{Free energy $t$-derivative: proof of identity \eqref{34}}\label{compDerivative}

Let us compute $\frac{df_{n,\epsilon}(t)}{dt}=\frac{1}{n}\mathbb{E}\big\langle\frac{d {\cal H}_{t,\epsilon}}{dt}\big\rangle_{t,\epsilon}$. Starting from \eqref{Ht}, \eqref{fnt} one obtains that $\frac{df_{n,\epsilon}}{dt}$ equals
%
\begin{align*}
\frac{1}{n}\mathbb{E}\Big\langle \lambda_nq_\epsilon(t)\sum_{i=1}^n\!\Big(\frac{x_i^2}{2} - x_iX_i-\frac{x_i\widetilde Z_i}{2\sqrt{R_\epsilon(t)}} \Big) - \lambda_n\sum_{i\le j}^n\!\Big(\frac{x_i^2x_j^2}{2n} - \frac{x_ix_jX_iX_j}{n}-\frac{x_ix_j Z_{ij}}{2\sqrt{n(1-t)\lambda_n}} \Big) \Big\rangle_{t,\epsilon}.
\end{align*}
%
Now we integrate by part the Gaussian noise using, as in the previous appendix, $\mathbb{E}[Zg(Z)]=\mathbb{E}\,g'(Z)$ for $Z\sim {\cal N}(0,1)$. This leads to
%
\begin{align*}
\frac{df_{n,\epsilon}}{dt}= \frac{\lambda_n}{n}\mathbb{E}\Big\langle q_\epsilon(t)\sum_{i=1}^n\Big(\frac{x_ix_i'}{2}- x_iX_i\Big)- \sum_{i\le j}^n\Big(\frac{x_ix_j x_i'x_j'}{2n}- \frac{x_ix_jX_iX_j}{n} \Big) \Big\rangle_{t,\epsilon}
\end{align*}
%
where $\bx$, $\bx'$ are two i.i.d. replicas drawn according to the posterior \eqref{tpost} (and thus share the same quenched variables). Slightly abusing notation, we continue to use the notation $\langle A(\bx,\bx')\rangle_{t,\epsilon}$ for the expectation w.r.t. the product measure $dP_{t,\epsilon}(\bx|\bW,\widetilde \bW)dP_{t,\epsilon}(\bx'|\bW,\widetilde \bW)$ of the i.i.d. replicas. An application of the Nishimori identities $\mathbb{E}[\langle x_i\rangle_{t,\epsilon} X_i] = \mathbb{E}\langle x_i x_i^\prime\rangle_{t,\epsilon}$ and $\mathbb{E}[\langle x_ix_j\rangle_{t,\epsilon} X_iX_j] = \mathbb{E}\langle x_ix_j x_i^\prime x_j^\prime\rangle_{t,\epsilon}$ then yields
%
\begin{align}
\frac{df_{n,\epsilon}}{dt}&= \frac{\lambda_n}{2}\mathbb{E}\Big\langle \frac{1}{n^2} \sum_{i\le j}^nx_ix_jX_iX_j -\frac{q_\epsilon(t)}{n}\sum_{i=1}^n x_iX_i  \Big\rangle_{t,\epsilon} \nonumber\\
&= \frac{\lambda_n}{2}\mathbb{E}\Big\langle  \frac{1}{2n^2} \sum_{i,j=1}^n x_ix_jX_iX_j +\frac{1}{2n^2} \sum_{i=1}^n x_i^2X_i^2 -\frac{q_\epsilon(t)}{n}\sum_{i=1}^n x_iX_i \Big\rangle_{t,\epsilon}\,. \label{last}
\end{align}
%
By Cauchy-Schwarz and the Nishimori identity $\mathbb{E}\langle \frac{1}{n^{2}}\sum_{i=1}^n x_i^2X_i^2\rangle_{t,\epsilon} =O(1/n)$. Indeed, by Cauchy-Schwarz
\begin{align*}
 \mathbb{E}\Big\langle \frac1n \sum_{i=1}^n x_i^2X_i^2\Big\rangle_{t,\epsilon} \leq 
 \Big\{\mathbb{E}\Big\langle \frac1n\sum_{i=1}^n x_i^4\Big\rangle_{t,\epsilon}\,\mathbb{E}\Big[\frac1n\sum_{i=1}^n X_i^4\Big]\Big\}^{1/2}= \mathbb{E}_{P_0}[X_1^4]\le 1
\end{align*}
where we used the Nishimori identity $\mathbb{E}\langle x_i^4\rangle_{t,\epsilon} = \mathbb{E}[ X_i^4]$ and the independence of the signal entries for getting the last equality. Expressing the two other terms in \eqref{last} with the help of the overlap $Q=\frac1n\sum_{i=1}^n x_iX_i$ gives \eqref{34}.

==> sections/all_or_nothing_XX.tex <==
\section{Phase transition threshold and matrix-MMSE}\label{sec:allOrNothing}
%
\begin{figure}[t]
\centering
\includegraphics[width=0.40\linewidth]{./figures/allornothing_Urademacher_matrixMMSE}
\includegraphics[width=0.40\linewidth]{./figures/allornothing_Vgaussian_matrixMMSE}

%\includegraphics[width=1.0\linewidth]{./plots/Plot_final}
 \caption{A sequence of matrix-minimum-mean-square-error (m-MMSE) curves as a function of $\lambda$ for the symmetric matrix estimation model. Here $\lambda_c(\rho) = 4\gamma \vert \ln \rho\vert$. In the sparse limit $\rho\to 0$ the curves approach a $0-1$ phase transition with the discontinuity at 
 $\lambda = \lambda_c(\rho)$.}
\label{fig:MMSEandMIWish}
\end{figure}
